Pump, Dump, and then What? The Long-Term Impact of Cryptocurrency Pump-and-Dump Schemes

The pump and dump scheme is a form of market manipulation attack in which coordinated actors drive up the price of an asset in order to sell at a higher price. Due in part to a lack of enforcement, these schemes are widespread within the cryptocurrency marketplace, but the negative impact of these events on the coins they target is not yet fully understood. Drawing upon a novel dataset of pump events extracted from Telegram channels, an order of magnitude larger than the nearest comparable dataset in the literature, we explore the differing tactics of pumping channels and the long-term impact of pump and dump schemes across 765 coins. We find that, despite a short-term positive impact in some cases, the long-term impact of pump and dump schemes on the targeted assets is negative, amounting to an average 30% relative drop in price a year after the pump event.

==> source/abstract.tex <==
Cryptocurrency pump and dump schemes involve the prices of coins being fraudulently inflated by an individual or a group of market participants before being sold off at a higher price, causing the value of the coin to significantly fall for any remaining investors.
These schemes are organised via social media sites such as Telegram and Discord which are used to coordinate the dates of pumps and the coins used.
To investigate the impact of these schemes, a new and enlarged dataset of around 10,000 pump events was produced by collecting data from organising channels on Telegram, as well as merging an existing dataset of 1,100 such events.
A comprehensive breakdown and performance analysis of the dataset reveals two distinct approaches to organising pump events, termed as the quality vs quantity tradeoff.
Investigating the pricing impact 365 days after pump events take place reveals an average 27\% decrease in the value of pumped coins relative to the wider market prices.
This represents conclusive evidence that pump events have a long-term negative impact on the value of pumped cryptocurrencies.
Finally the impact of FTX's collapse on pump events is explored which reveals no direct material impact on the number of pumps organised.
However, the wider fall in prices of coins and lower volumes moved during pumps decreases the potential amount of money that operators, and to a lesser extent participants, could potentially make.

==> source/background.tex <==
%This chapter is intended to describe the background on which execution of the project depends. This may be a technical or a contextual background, or both. The goal is to provide a detailed explanation of the specific problem at hand, and existing work that is relevant (e.g., an existing algorithm that you use, alternative solutions proposed, supporting technologies).
%
%Per the same advice in the handbook, note there is a subtly difference from this and a full-blown literature review (or survey).  The latter might try to capture and organise (e.g., categorise somehow) \emph{all} related work, potentially offering meta-analysis, whereas here the goal is simple to ensure the dissertation is self-contained.  Put another way, after reading this chapter a non-expert reader should have obtained enough background to understand what \emph{you} have done (by reading subsequent sections), then accurately assess your work against existing relevant related work.  You might view an additional goal as giving the reader confidence that you are able to absorb, understand and clearly communicate highly technical material and to situate your work within existing literature.












==> source/background/introduction_to_crytpocurrencies.tex <==
\subsection{A Mutually Exclusive Relationship}
\label{subsec:cryptocurrencies-introduction}
This section explores what cryptocurrencies are and their relationship with the current lack of regulations.
It then introduces encrypted anonymous social media and how these all intersect to create the conditions for large-scale pump and dump schemes.


\subsubsection{One Man and His Dream}
\label{subsubsec:one-man-and-his-dream}
Cryptocurrencies (also referred to as coins) are digital representations of value that, in general, do not have a physical form in the same way that traditional currencies do.
The ownership of these coins is stored digitally in wallets and transactions are carried out via a distributed ledger, the most common type of which is a blockchain~\cite{UK-gov-crypto-def-2023}.
The most well known and first example of a cryptocurrency is Bitcoin, which was created in 2009 to facilitate peer-to-peer irreversible electronic transactions that were independent of existing financial institutions~\cite{nakamoto-bitcoin-2008}.

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.45\textwidth]{background/cryptocurrency_count}
    \caption{Number of cryptocurrencies from 2013 to 2023 listed on CoinMarketCap~\cite{statistica-count-2023}.}
    \label{fig:crypto_count}
\end{figure}

Since 2009 the number of cryptocurrencies has vastly increased\footnote{Whilst this has decreased since the start of 2022, the total number is still far greater than is was in 2009.}, as shown in Figure~\ref{fig:crypto_count}, and as of February 2023 there were 8,685 active cryptocurrencies listed on CoinMarketCap\footnote{\url{https://coinmarketcap.com}, a website that provides aggregated price data for cryptocurrencies.}.
These cryptocurrencies are known as alternative coins or ``altcoins'' by the nature of being alternatives to Bitcoin.
The majority of these have a low market capitalisation, a measure of a cryptocurrency's value\footnote{See Section~\ref{subsubsec:market-capitalisation} for more detail on market capitalisation.}, and are not widely traded.
The top 5 coins account for $71.86\%$ of total market capitalisation as of 6 February 2023~\cite{coingecko-market-cap-2023}.
This leaves the majority of cryptocurrencies with little or no market capitalisation, implying they have minimal value and are not widely traded.


\subsubsection{The Current (Non-)State of Regulation}
\label{subsubsec:the-current-state-of-regulation}
Pump and dump schemes are considered market manipulation with respect to the stock market and traded securities in the U.S.~\cite{securities-exchange-act-1934} and infringements are actively enforced by the SEC\@.
For example in December 2022 the SEC charged 8 influencers with market manipulations for a $\$100$ million scheme that involved promoting stocks to pump and dump them~\cite{sec-market-charge-2022}.
This sort of enforcement action, however, is not present with respect to pump and dump schemes in the cryptocurrency sphere.
Research by Corbet et al$.$ found that Bitcoin, and other cryptocurrencies, do not effectively fit into any existing SEC framework for regulation~\cite{corbet-regulation-2021} implying that enforcement action relating to market manipulation cannot be taken with respect to cryptocurrencies.
This is further backed up by remarks made by William Hinman\footnote{The director of corporate finance at the SEC from 2017 to 2020.}, who stated that the SEC does not consider a cryptocurrency to be a security if it is deemed ``sufficiently decentralised''~\cite{hinman-remarks-2018}, indicating that existing rules regarding market manipulation of securities are not applicable to most cryptocurrencies as they typically rely on a decentralised ledger.


\subsubsection{Digging a Big Hole}
\label{subsubsec:digging-a-big-hole}
Up until this point a lack of regulation for cryptocurrencies appears not to have been a problem given that their original purpose was to be decentralised, trustless and crucially outside the control of existing central authorities and their respective regulations~\cite{nakamoto-bitcoin-2008}.
The problem with this system is that transactions need to be irreversible in order to be trustless, requiring transactions to be authenticated in a way such that they cannot be reversed.
This is commonly achieved through a practice known as ``mining'', where an intermediary solves a resource intensive task in order to validate transactions and in return receives a reward for doing so.
The reason for the task being resource intensive is to make it computationally impossible for a malicious actor to acquire enough resources to outnumber benign actors and validate invalid transactions~\cite{mukhopadhyay-mining-2016}, in effect guaranteeing the trustlessness of the system.


\subsubsection{Exchanging It Up}
\label{subsubsec:exchanging-it-up}
There is, unfortunately, a fundamental flaw with this system caused by the time it takes to perform these authentication tasks, which on average took 7.24 minutes in the period spanning February 2022 to February 2023~\cite{blockchain-time-2023}.
This incredibly long timeframe, especially compared to modern securities and FX markets, means that the blockchain on its own it is not an attractive option for participants used to near real time transaction execution.
The solution to these problems comes in the form of cryptocurrency exchanges, which are platforms that function in a similar way to traditional banks and electronic securities trading platforms.
These allow users to easily buy and sell coins in real time by interfacing with a centralised exchange that acts as a broker between the participant and the blockchain as well as providing secure storage for users' coins without requiring participants to understand how the underlying blockchain functions.

Exploring cryptoexchanges has exposed a number of contradictions with the original design and purpose of cryptocurrencies, chief among these are their centralisation and requirement for the participant to trust them with their money.
This centralisation means that the exchange is a single point of failure and attack, effectively functioning as a bank.
Traditional banks have significant regulatory oversight and requirements, yet cryptoexchanges do not~\cite{chohan-ftx-2023}, which is an issue that has the potential to become a significant problem\footnote{See Section~\ref{subsubsec:the-perfect-storm-in-the-wild-west}.}.


\subsubsection{Telegram Enters the Chat}
\label{subsubsec:the-role-of-telegram}
Telegram is a cloud-based messaging app that claims to combine speed and security~\cite{telegram-claims-2023}.
It has become a hub for cybercriminals due to its light touch moderation and features such as one-way broadcast channels and encrypted direct messaging as well as being simpler to use than the dark web, the traditional marketplace for clandestine activities~\cite{ft-telegram-2021}.
These channels allow admins to broadcast messages to a large audience (in some examples into the hundreds of thousands) of subscribers whilst not displaying the sender's identity or allowing such subscribers to respond directly to the message.
Combining this with the perceived anonymity of the platform and a general absence of moderation, especially compared to other social media platforms makes Telegram an ideal platform for announcing and coordinating pump and dump schemes.


\subsubsection{Storms in the Wild West}
\label{subsubsec:the-perfect-storm-in-the-wild-west}
As discussed in Section~\ref{subsubsec:the-current-state-of-regulation}, the general lack of applicable regulation to cryptocurrencies have been termed the ``wild west'' by Gary Gensler, the chair of the SEC~\cite{gensler-remarks-2021}.
This in combination with the mass messaging features of Telegram channels as well as a large variety of virtually unknown cryptocurrencies with low volumes and market capitalisation (see Section~\ref{subsubsec:one-man-and-his-dream}) has created the perfect storm for pump and dump schemes to flourish.

A further example of just how ``wild'' the cryptocurrency sphere is was evidenced by the collapse of FTX, where the exchange was allowed to funnel customer deposits into its own trading firm~\cite{chohan-ftx-2023}, creating a $\$10$ billion black hole in its finances, eventually leading to its collapse in November 2022.
The fact that cryptoexchanges are not bound by traditional banking laws and regulations and a lack of specific regulation for cryptoexchanges enabled fraud on an epic scale to occur, costing retail investors at least $\$1$ billion~\cite{reuters-ftx-2022}.
The collapse also caused big shocks in the market and has eroded the confidence of retail investors, the main participants in pump and dump schemes, in cryptocurrencies, in effect reducing the attractiveness of these schemes as investors become more risk averse.

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.4\textwidth]{background/ftx_impact}
    \caption{An attempt by a pump organiser to reassure participants after the collapse of FTX.}
    \label{fig:ftx-impact-message}
\end{figure}

A direct example of such an impact is shown in Figure~\ref{fig:ftx-impact-message}, where a pump organiser attempts to reassure participants that the collapse of FTX will not affect the profitability of future pumps.
This indicates that the collapse FTX had an impact on the operations of these pump and dump schemes, and will be used as an analytical component later in this thesis.

==> source/background/pump_dump_mechanics.tex <==
\subsection{Mind, Body and Soul - the Anatomy of a Pump and Dump}
\label{subsec:mechanics-of-a-pump-and-dump-scheme}
The mechanics of pump and dump were first described by Xu and Livshits~\cite{xu-anatomy-2019} and consist of multiple phases coordinated through a Telegram channel.
In general these are the pre-pump announcement, the pumping phase, the dumping phase and the post-pump analysis.

\paragraph{Pre-pump announcement.}
These messages are used to advertise the date and time of the next pump as well as the exchange upon which the pump will take place.
There are typically multiple messages posted in the channel in the weeks and days leading up to the pump and usually come with marketing messages to encourage members to take part.

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.35\textwidth]{background/inital_pump_announcement}
    \caption{Example of an inital pre-pump announcement.}
    \label{fig:inital_pump_announcement}
\end{figure}

Figure~\ref{fig:inital_pump_announcement} shows an example of an initial pre-pump announcement, stating the date, time and exchange for next pump.

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.35\textwidth]{background/30_min_pre_pump}
    \caption{Example of a pre-pump reminder.}
    \label{fig:30_min_pump_announcement}
\end{figure}

Figure~\ref{fig:30_min_pump_announcement} shows an example of a reminder that are sent to the channel right before the pump and highlights how channel admins attempt to hype up the pump before it begins.


\paragraph{Pumping phase.}
The pumping phase begins with a message announcing the coin that is going to be pumped, an example of which is shown in Figure~\ref{fig:pump_start}.

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.3\textwidth]{background/pump_start}
    \caption{Example message annoucing the start of a pump.}
    \label{fig:pump_start}
\end{figure}

This initial message is typically followed by more messages from the channel admins encouraging members to continually buy the coin and hold it.


\paragraph{Dumping phase.}
There is rarely any signal from the organisers to sell coins and instead they continue to encourage members to buy more in dips meaning the decision to sell is left up to the participants themselves.
This means that as soon as the price of the coin starts to fall, participants begin to rapidly panic and sell off their coins as they fear losing money, causing the price of the coin to collapse.


\paragraph{Post-pump analysis.}
Channel admins often post post-pump results to advertise how much money participants could have made if they had sold the coin at the peak of the pump, relative to the price of the coin before the event, an example of which is shown in Figure~\ref{fig:post_pump_analysis}.

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.3\textwidth]{background/post_pump_analysis}
    \caption{Example message providing post pump analysis.}
    \label{fig:post_pump_analysis}
\end{figure}

The statistics given in these are selectively chosen to make the pump appear as successful as possible.
This makes the pumps appear as attractive as possible for new members of the channel.
The profit figures quoted by such posts rarely represent the actual profit, if any, made by participants since achieving the quoted figures requires participants to sell their coins in a window that can be as short as tenths of a second.

==> source/definitions.tex <==
The following acronyms and abbreviations are used throughout this thesis:

\begin{quote}
    \noindent
    \begin{tabular}{lcl}
        CCXT & : & CrytoCurrency eXchange Trading library. \\
        SEC & : & Securities and Exchange Commission. \\
        U.S.\ & : & United States of America. \\
        OHLCV & : & Open, High, Low, Close, Volume. \\
        RF & : & Random Forest. \\
        GLM & : & Generalised Linear Model. \\
        CEX & : & Centralised Exchange. \\
        DEX & : & Decentralised Exchange. \\
        XGBoost & : & Extreme Gradient Boost. \\
        LSTM & : & Long Short-Term Memory. \\
        CAR & : & Cumulative Abnormal Returns. \\
        \verb|regex| & : & Regular Expressions. \\
        API & : & Application Programming Interface. \\
        KYC & : & Know Your Customer. \\
        CPI & : & Crypto Pump Island. \\
        IQR & : & Interquartile Range.
    \end{tabular}
\end{quote}

==> source/evaluation/overview.tex <==
\subsection{Overview}
\label{subsec:analysis-overview}
The analysis phase of the project analyses the collected data and is focused on four areas.

\begin{itemize}
    \item \textbf{Dataset Breakdown (Section~\ref{subsec:dataset-analysis-and-breakdown}).}
    Initial dataset breakdown and trend highlighting.
    \item \textbf{Pump Performance (Section~\ref{subsec:pump-performance}).}
    Investigation into pump performance.
    \item \textbf{Long-term Impacts (Section~\ref{subsec:long-term-impacts}).}
    Long-term price impacts relative to the general markets.
    \item \textbf{Collapse of FTX (Section~\ref{subsec:the-collapse-of-ftx}).}
    Effects and fallout from the collapse of FTX\@.
\end{itemize}

The overarching aim of this chapter is to provide unique insights to the collected dataset and to answer the main hypothesis of this project.

==> source/evaluation/tables/cpi_proportion.tex <==
\begin{table}[!htbp]
    \centering
    \caption{Pumps separated by organiser before and after FTX.}
    \label{tab:proportion_cpi_ftx}
    \begin{tabular}{lrrrr}
        \toprule
        {} & \multicolumn{2}{c}{\textbf{CPI}} & \multicolumn{2}{c}{\textbf{Others}} \\
        {} &   Number &  Proportion &  Number &  Proportion \\
        \midrule
        Before &  7623 &           87.37 &     297 &              63.73 \\
        After  &  1102 &           12.63 &     169 &              36.27 \\
        \midrule
        \textbf{Total} & \textbf{8725} & {} & \textbf{466} & {} \\
        \bottomrule
    \end{tabular}
\end{table}


==> source/evaluation/tables/deltas.tex <==
\begin{table}[!htbp]
    \centering
    \caption{The longest avaliable timeframe for CPI and non-CPI organised pumps.}
    \label{tab:deltas}
    \begin{tabular}{lrrrrrr}
        \toprule
        {} & \multicolumn{3}{c}{\textbf{CPI}} & \multicolumn{3}{c}{\textbf{Others}} \\
        \textbf{Timeframe} & Number & Percentage & Cumulative & Number & Percentage & Cumulative \\
        \midrule
        1 hour       &       27 &    0.34 &         0.34 &           4 &      0.31 &            0.31 \\
        6 hours      &       48 &    0.61 &         0.95 &           9 &      0.71 &            1.02 \\
        12 hours     &      168 &    2.12 &         3.07 &           9 &      0.71 &            1.73 \\
        1 day        &      291 &    3.67 &         6.74 &           9 &      0.71 &            2.44 \\
        2 days       &      979 &   12.36 &        19.10 &          61 &      4.80 &            7.24 \\
        5 days       &      546 &    6.89 &        25.99 &          31 &      2.44 &            9.68 \\
        1 week       &     1320 &   16.67 &        42.66 &         140 &     11.01 &           20.69 \\
        2 weeks      &     1600 &   20.20 &        62.86 &         191 &     15.03 &           35.72 \\
        1 month      &     1389 &   17.54 &        80.40 &         146 &     11.49 &           47.21 \\
        2 months     &      613 &    7.74 &        88.14 &         130 &     10.23 &           57.44 \\
        3 months     &      600 &    7.58 &        95.72 &         196 &     15.42 &           72.86 \\
        6 months     &      170 &    2.15 &        97.87 &          82 &      6.45 &           79.31 \\
        9 months     &       70 &    0.88 &        98.75 &          91 &      7.16 &           86.47 \\
        1 year       &       99 &    1.25 &          100 &         172 &     13.53 &             100 \\
        \midrule
        \textbf{Total} & \textbf{7920} & {} & {} & \textbf{1271} & {} & {} \\
        \bottomrule
    \end{tabular}
\end{table}


==> source/evaluation/tables/diff_full_others.tex <==
\begin{table}[!htbp]
    \centering
    \caption{Summary of long-term impacts of CPI and non-CPI organised pumps, grouped by number of pumps and averaged using the IQR mean.}
    \label{tab:diff_full_cpi}
    \addtolength{\tabcolsep}{-0.4em}
    \begin{tabular}{lrrrrrrrr}
        \toprule
        Days & \textbf{7} & \textbf{14} & \textbf{30} & \textbf{60} & \textbf{90} & \textbf{180} & \textbf{270} & \textbf{365} \\
        \midrule
        1 & 93.85 & 94.45 & 92.88 & 85.16 & 79.76 & 74.02 & 71.61 & 79.13 \\
        2+ & 96.55 & 94.45 & 88.27 & 87.50 & 73.00 & 73.67 & 74.78 & 66.76 \\
        \bottomrule
    \end{tabular}
\end{table}


==> source/evaluation/tables/diff_subset_others.tex <==
\begin{table}[!htbp]
    \centering
    \caption{Summary of long-term impacts of CPI and non-CPI organised pumps for coins on their 1st to 4th pumps, averaged using the IQR mean.}
    \label{tab:diff_subset_cpi}
    \addtolength{\tabcolsep}{-0.4em}
    \begin{tabular}{lrrrrrrrr}
        \toprule
        Days & \textbf{7} & \textbf{14} & \textbf{30} & \textbf{60} & \textbf{90} & \textbf{180} & \textbf{270} & \textbf{365} \\
        \midrule
        1 & 94.76 & 94.45 & 91.33 & 85.84 & 77.36 & 73.88 & 72.93 & 73.38 \\
        2 & 98.08 & 98.43 & 94.42 & 89.12 & 77.76 & 86.19 & 73.63 & 75.64 \\
        3 & 100.05 & 101.08 & 95.25 & 85.29 & 64.68 & 89.07 & 73.95 & 73.90 \\
        4 & 97.58 & 98.84 & 95.53 & 94.28 & 65.98 & 95.21 & 90.43 & 92.17 \\
        \bottomrule
    \end{tabular}
\end{table}

